Towards Measuring Microlensing Event Rate in the Galactic Center: I. Events Detection from the UKIRT Microlensing Survey Data

To overcome the high optical extinction, near-infrared observations are needed for probing the microlensing events toward the Galactic center. The 2015-2019 UKIRT microlensing survey toward the Galactic center is the first dedicated precursor near-infrared (NIR) survey for the Nancy Grace Roman Space Telescope. We here analyze the online data from the UKIRT microlensing survey, reaching $l=b=0^\circ$. Using the event-finder algorithm of KMTNet with the $\Delta \chi^2$ threshold of 250, we find 522 clear events, 436 possible events, and 27 possible anomalous events. We fit a point-source point-lens (PSPL) model to all the clear events and derive the PSPL parameters with uncertainties using a Markov chain Monte Carlo method. Assuming perfect detection efficiency, we compute the uncorrected event rates, which should serve as the lower limits on the true event rate. We find that the uncorrected NIR event rates are likely rising toward the Galactic center and higher than the optical event rates.

==> backup <==


\section{Introduction} \label{sec:intro}
%write my introduction right here...
Since the first planet detected via microlensing two decades ago \citep{Bond04}, microlensing has established itself as an important technique for exoplanet detection and characterization. Planets are discovered by their gravitational perturbation of light from a more distant source. The technique can be used to search for planets orbiting host stars with a broad range of masses and distances \citep{Gaudi12}. 
%It is sensitive to very low-mass planets on wide orbits, an
It is sensitive to very low-mass planets on wide orbits around the so called Einstein ring radius \citep{Mao91, Andy1992, Bennett1996}. 
For typical Galactic microlensing events, the Einstein ring radius is 2 to 3 times the snow line radius. Thus the microlensing survey can provided important constraints on the demographics of planets beyond the snow line \citep{Zang22}. 
For example, previous surveys have found that planets near and beyond the snowline are abundant, with an occurrence frequency in the range of $\sim 50\%$ to $100\%$ \citep{Gould10,Cassan2012,Wise,Suzuki2016}. \citet{Suzuki2016} found a break in the mass function of smaller microlensing planets, which would have important implications for the formation of cold planets \citep{Suzuki2018, Deng21} and brown dwarfs  \citep{ma14, Poleski17, feng22, Bachelet22} around solar-type stars.
Besides, microlensing is currently the only technique that can systematically probe the free-floating planet population \citep{Sumi11}. 
%diagnostics
% formation and evolution 
% \citet{Suzuki2016} studied a sample of 23 planets detected by the MOA-II survey (2007--2012) and found that microlensing planets more frequently have smaller planet to host mass ratios, $q$, until the trend reverses at $q \sim 57q_{\oplus}$, where $q_{\oplus} = 3 \times 10^{-6}$ is the mass ratio of Earth/Sun. 
% This turn over was not expected in the standard core accretion theory \citep[e.g.,][]{Ida2004} and would have important implications for the formation of cold planets \citep{Suzuki2018, Deng2021formation} and brown dwarfs  \citep{ma14, Poleski17, feng22}.


% The ability of a microlensing experiment to detect these systems relies heavily on the underlying microlensing event rate, which itself depends on the surface density of source and lens stars toward the survey fields. Therefore, microlensing surveys have concentrated their observing efforts toward the Galactic bulge, where the stellar surface density is highest. However, tra- ditionally these surveys have been conducted in optical wavelengths, which suffer from high extinction near the Galactic plane and center, and thus their fields were selected in order to balance the stellar surface density with the extinction.

%Popowski et al. (2001) proposed that optical depth may be estimated without any bias due to blending by using only events with bright source stars, such as red clump giants (RCGs), in which the blending might be negligible, rather than using all sources including the faint sources as in previous studies. Except for one high value measured by Alcock et al. (1997), the other measurements based on events with bright sources resulted in lower optical depths when measured by EROS (Afonso et al. 2003), MACHO (Popowski et al. 2005), and EROS (Hamadache et al. 2006).


%The event rate per star per year Γ i
The ability of a survey to detect microlensing events depends heavily on the event rate per star per year $\Gamma$, which itself depends on the surface density of source and lens stars in the survey field. 
Thus knowing the event rate distribution in that direction is crucial for experiment design of various microlensing survey program, like $\it{CSST}$, $\it{Roman}$ and $\it{ET2.0}$ \citep{Spergel2015, Ge22}. 
Furthermore, the event rate can reveal information about the structure of the bulge \citep[e.g.,][]{Kiraga94}, and the connection between statistics of microlensing events and the Galactic bulge structure is an area of active research \citep{Kerins09, Sumi13, Wyrzykowski15, Awiphan16, Portail17, Barbuy18, Lam20, Koshimoto21, Winch22}. 
% %Additionally, the event rate gives us information about the structure of the bulge
% (e.g., Kiraga & Paczy´nski 1994). The connection between statistics of observed events and
% the structure of the bulge is an area of active research (Kerins et al. 2009; Sumi et al. 2013;
% Wyrzykowski et al. 2015), but a full understanding of microlensing event rate has not yet
% been achieved.
However, optical microlensing surveys are usually restricted from detecting events near the Galactic plane and center, where the event rate is considered to be the highest due to the high optical extinction \citep{Gould95, Shvartzvald18, Navarro18, Bennett18, Penny19, Wyrzykowski22}. 
\citet{Sumi13} and \citet{Sumi16} measured the optical depths and event rates near the $b=-1^\circ.4$ region by analyzing $\sim500$ MOA events from the 2007 and 2008 seasons, and found the event rate is increasing toward the bulge center. \citet{Penny19} confirmed this trend using a suite of Galactic model simulations.
%Currently the study measuring optical depths and event rates with the largest number of events analyzes $\sim500$ MOA events from the 2007 and 2008 seasons . 
%(Sumi et al. 2013; Sumi & Penny 2016).
%Navarro18: We find a slight asymmetry, with a larger number of events toward negative longitudes than positive longitudes. This asymmetry is seen both in the complete sample and the subsample of RC giant sources, and it is possibly related with the inclination of the bar along the line of sight. The timescale distribution is fairly symmetric with a peak in 19.6 ± 1.1 days for the complete sample (N = 630 events), and 20.7 ± 1.0 days for the RC stars (N = 291 events), in agreement with previous results.
In order to penetrate the dust near the Galactic plane and reach sources throughout the bulge and into the far side of the Galactic disk, an infrared microlensing survey is required. 
\citet{Shvartzvald17} started another campaign using the the United Kingdom Infrared Telescope (UKIRT) located at Mauna Kea Observatory to facilitate a preliminary estimation of the NIR event rate per source $\Gamma$ toward the Galactic center. 
VISTA Variables in the Via Lactea (VVV) conducted a variability survey toward the inner Milky Way in the NIR \citep{Navarro18, Alonso18}, where they give a typical event timescale of $\sim20$~days. 
\citet{Navarro20} studied for the first time the microlensing events latitude distribution reaching $b=0^\circ$ in the Galactic center using the VVV survey data. They found the events number increase rapidly from $b=2^\circ$ to $b=0^\circ$ by an order of magnitude, with a slope much stepper than that along the Galactic longitude. 

%Koshimoto 21
% %Weestimate various fundamental model parameters for our Galaxy through our modeling, including the initial mass
% function (IMF) in the inner Galaxy. Combined constraints from star counts and the microlensing event timescale
% distribution from the OGLE-IV survey, in addition to a prior on the bulge stellar mass, enable us to successfully
% measure IMF slopes using a broken power-law form over a broad mass range

To the best of our knowledge, there is no microlensing event rate estimation in the Galactic center near the $l=b=0^\circ$ region. 
VVV and UKIRT surveys are currently the only two experiments with the ability to probe this region. Here we analyze the UKIRT microlensing survey data from 2015-2019 and present the detection of microlensing events discovered by the survey in this Paper I. 
%, and estimate the preliminary event rate toward its survey fields. 
%This work provides the best estimate of the event rate in the inner GB to date.
%and microlensing optical depth
We describe the observation and the survey data in Section~\ref{sec:Observations}. In Section~\ref{sec:method}, we present the microlensing events detection algorithm and the results. Finally we discussion the implication of our results for future microlensing surveys in Section~\ref{sec:discussion} and give a conclusion in Section~\ref{sec:conclusion}.
